Learning Human-to-Robot Handovers from Point Clouds

We propose the first framework to learn control policies for vision-based human-to-robot handovers, a critical task for human-robot interaction. While research in Embodied AI has made significant progress in training robot agents in simulated environments, interacting with humans remains challenging due to the difficulties of simulating humans. Fortunately, recent research has developed realistic simulated environments for human-to-robot handovers. Leveraging this result, we introduce a method that is trained with a human-in-the-loop via a two-stage teacher-student framework that uses motion and grasp planning, reinforcement learning, and self-supervision. We show significant performance gains over baselines on a simulation benchmark, sim-to-sim transfer and sim-to-real transfer.

==> sections/tables/table_rebuttal.tex <==
\begin{table}[t]
 \vspace{-0.2cm}
 \centering
 \small
 % \setlength{\tabcolsep}{6pt}
  \resizebox{0.9\columnwidth}{!}{%
 \begin{tabular}{l|cccc}
%   \hline
%   \multicolumn{5}{c}{Ablation Study} \\
%   \hline
  \multirow{2}{*}{HandoverSim benchmark} & \multirow{2}{*}{success (\%)} &  \multicolumn{3}{c}{failure (\%)} \\
  & & contact & drop & timeout \\
  \hline

   w/ RGBDM + ResNet18 & 34.10  & ~~\textbf{6.20} &  45.80     &  13.90          \\
  \rowcolor{Gray}
   w/ Kinect noise & 59.49 & 13.19 &  19.68 &  ~~7.64         \\ 


   w/ third person view & 60.42  & ~~9,95 &  25.69     &  ~~3.94          \\
     \rowcolor{Gray}
   w/o aux prediction & 70.60  & 10.65 &  16.20     & ~~2.54          \\

 

  \textbf{Ours} & \textbf{75.23} & ~~9.26 & \textbf{13.43} & ~~\textbf{2.08} \\ \hline

 \end{tabular}
 }
 \vspace{-2mm}
 \caption{\textbf{Ablation.} We ablate the our method's vision components and the auxiliary loss. Results are averaged over 3 random seeds.
%  \wei{Refer ``RGBDM" in the main text?}
 }
 \vspace{-4mm}
 \label{tab:rebuttal}
\end{table}

==> sections/tables/table_sim2sim.tex <==
\begin{table*}[t]
 % \vspace{-2mm}
 \centering
 \small
 % \setlength{\tabcolsep}{6pt}
 \begin{tabular}{l|l|cccc|cccc}
  \hline
  \multicolumn{9}{c}{Sim-to-Sim} \\
  \hline
  & & \multirow{2}{*}{success (\%)} & \multicolumn{3}{c|}{mean accum time (s)} & \multicolumn{4}{c}{failure (\%)} \\
  & & & exec & plan & total & contact & drop & timeout & total \\
  \hline
  \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Sequential}}}
%   & OMG Planner~\cite{wang:rss2020}        & 58.33 & 8.304          & ~~2.486          &  10.790          &  32.64          & ~~\textbf{7.64} & ~\textbf{1.39} \\
%   & \gc Yang et al.~\cite{yang:icra2021} & \gc 56.25  & \gc \textbf{4.414}  & \gc ~~0.617          & \gc 5.031          &  \gc 16.67          &  \gc 18.06          & \gc ~~9.03          \\
  & GA-DDPG~\cite{wang:corl2021b} &  19.44          & ~7.171          & ~0.175          & ~7.346          & \textbf{4.86} & 47.22          & 28.47   &   80.56    \\
  & \gc GA-DDPG~\cite{wang:corl2021b} finetuned  & \gc tbd         & \gc tbd        & \gc tbd & \gc tbd      & \gc tbd &  \gc tbd          &  \gc tbd    & \gc tbd    \\
  
  &  Ours & 44.21 & 7.666 & 0.236 & 7.901  & 9.49 & 40.51 & 5.79 & 55.79  \\ 
  
  & \gc Ours w/o grasp & \gc \textbf{54.40} & \gc 9.165 & \gc 0.239 & \gc 9.403  & \gc 7.87 & \gc \textbf{33.34} & \gc \textbf{4.40} & \gc \textbf{45.60} \\
%   Ours (hand avg + pred)  w/o hold & 43.73 & tbd & tbd & tbd  & 16.3 & ~21.5 & ~18.40 \\ 
 

  \hline

  \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Simult.}}}
  
  & GA-DDPG~\cite{wang:corl2021b} & 11.11          & \textbf{4.678} & ~\textbf{0.168}          & ~\textbf{4.847} & 15.97          & 48.61          & 24.31  & 88.89        \\
  & \gc GA-DDPG~\cite{wang:corl2021b} finetuned  & \gc tbd          & \gc tbd          & \gc tbd & \gc tbd         & \gc tbd &  \gc tbd          & \gc tbd & \gc tbd      \\
 
  & Ours    & 39.58 & 6.129 & 0.220 & 6.349  & 9.03 & 43.75  & 7.64 & 60.42   \\
  & \gc Ours w/o grasp pred. & \gc \textbf{47.92} & \gc 7.610 & \gc 0.222 & \gc 7.833  & \gc \textbf{10.65} & \gc \textbf{35.88} & \gc \textbf{5.56}  & \gc \textbf{52.08} \\ 
  
\bottomrule
  
 \end{tabular}
 % \vspace{-2mm}
 \caption{\textbf{Sim-to-Sim experiment}. We evaluate sim-to-sim transfer of the learning-based methods, i.e., we train policies in Pybullet \cite{kalevatykh:2020} and evaluate them in Isaac Gym\cite{makoviychuk:neuripstdb2021}. We find that our method has much better transfer capabilities than GA-DDPG \cite{wang:corl2021b}, in both the sequential and the simultaneous setting. Closer analysis indicates that part of the performance drop of our method is caused by the grasp prediction policy not transferring well, which we see when comparing 'Ours' against 'Ours w/o grasp pred.'. Results are averaged across 3 random seeds.}
 % \vspace{-2mm}
 \label{tab:sim2sim}
\end{table*}

==> supp_sections/04_limitations.tex <==
\section{Limitations and Future Work}
\label{app_lim}

We will now discuss failure cases of our method and exciting directions for future work. Some failures occur with smaller objects, where the human hand often encloses large parts of the object. For the robot to find grasps where the gripper does not touch the hand at all in such cases is extremely difficult, especially when only having access to point cloud input. The grasp prediction task that decides when to switch from approaching to grasping is quite challenging, because a small change in end-effector pose can already cause a handover to fail. We sometimes find that the grasp prediction triggers the grasp too early or in an instance where the object will eventually drop. Since the grasp prediction network is trained offline, it may be improved by finetuning in online fashion with experiences from policy rollouts. Furthermore, we investigate \textit{sensor-challenging} objects in real world transfers. Our depth sensor is vulnerable to transparent or dark objects, which may lead to failures of the policy (\Fig{real_failure}). Improving the vision pipeline to detect such objects reliably \cite{yen:2022icra} could be a viable direction.

We find that most human trajectories in HandoverSim have roughly the same length. A future direction can therefore include exploring a wider variety of human behaviors. \update{For example, in a realistic, interactive setting the human may be constantly moving, and the robot should only take objects from the human once it wants to hand them over. Anticipating the intent and future states of the human could provide a more natural system. We also noticed that humans start adapting to the robot once they learn how it behaves. Therefore, introducing a multi-agent training scheme where both the simulated human and the robot are trained jointly \cite{langerak2022marlui} is interesting. Another direction could include making the RL exploration more efficient, as it currently still requires long training times, e.g., by leveraging state-agnostic priors \cite{bagatella2022sfp} or using an intrinsic reward to incentivize contacts \cite{vulin2021}. Lastly, our framework can potentially serve as a real world application framework to evaluate vision pipelines, e.g., for testing hand and object pose estimation estimation pipelines \cite{ziani2022tempclr,tse2022collaborative} or segmentation models \cite{fan2021digit}.}

% \columnbreak

\makeatletter
\setlength{\@fptop}{0pt}
\makeatother
\input{supp_sections/supp_images/real_world_limitation}

% \onecolumn
% \twocolumn



==> supp_sections/05_glossary.tex <==
\section{Glossary}
\label{app_glossary}

